AutoDIAL: Automatic DomaIn Alignment Layers

Classifiers trained on given databases perform poorly when tested on data acquired in different settings. This is explained in domain adaptation through a shift among distributions of the source and target domains. Attempts to align them have traditionally resulted in works reducing the domain shift by introducing appropriate loss terms, measuring the discrepancies between source and target distributions, in the objective function. Here we take a different route, proposing to align the learned representations by embedding in any given network specific Domain Alignment Layers, designed to match the source and target feature distributions to a reference one. Opposite to previous works which define a priori in which layers adaptation should be performed, our method is able to automatically learn the degree of feature alignment required at different levels of the deep network. Thorough experiments on different public benchmarks, in the unsupervised setting, confirm the power of our approach.

==> intro_bk.tex <==
%Many scientists today believe we are witnessing the golden age of computer vision. 
In the past few years research in computer vision has seen a lot of progress, The massive adoption of machine learning and, in particular, of deep learning techniques as well as the availability of large fully annotated datasets have enabled amazing advances in the field.
A natural question is if the novel generation of computer vision technologies is robust enough to operate in real world scenarios.
One of the main problems is that the central assumption that training and test data are independently and identically drawn from the same distribution does not hold in many real world applications.
Indeed, researchers have shown that, even with powerful deep learning models, the so-called domain shift problem can be alleviated but not eliminated \cite{donahue2014decaf}.
Therefore, solving this issue represents a fundamental challenge for developing computer vision systems working in the real world.

In the last few years the research community has devoted significant efforts in addressing domain shift, and several methods for domain adaptation have emerged.
Domain adaptation focuses on improving learning performance in a target task by
leveraging knowledge from a related source task.
In this context, the specific problem of unsupervised domain adaptation, \ie no labeled data are available in the target domain, deserves special attention, as in many applications annotating data is not only a tedious operation but may be not possible.

Several approaches have been proposed for unsupervised domain adaptation in the past, both considering hand-crafted features~\cite{huang2006correcting,gong2013connecting,gong2012geodesic,long2013transfer,fernando2013unsupervised} and deep models~\cite{long2015learning,tzeng2015simultaneous,ganin2014unsupervised,long2016unsupervised,ghifary2016deep,li2016revisiting}.
%Among recent works based on convolutional neural networks (CNN), feature alignment methods have achieved remarkable performance. Feature alignment approaches aim to discover a new feature representation for the source and target domain in order to reduce the discrepancy among data distributions. Two strategies are typically employed for aligning source and target distributions. One strategy is based on the minimization of Maximum Mean Discrepancy (MMD) \cite{long2015learning,long2016unsupervised}, \ie additional layers are introduced in the network to force the distributions of the learned source and target representations to be as similar as possible in MMD terms. A second strategy \cite{tzeng2015simultaneous,ganin2014unsupervised} is based on the introduction of a domain-confusion loss. This loss is used to learn an auxiliary classifier predicting if a sample comes from the source or the target domain. Intuitively, by maximizing this term, \ie by imposing the auxiliary classifier to exhibit poor performance, domain-invariant features are learned.
In particular, recent works based on convolutional neural networks (CNN) have achieved remarkable performance.
Most of these methods attempt to reduce the discrepancy among source and target distributions by learning features that are invariant to the domain shift.
Two main strategies are typically employed.
One is based on the minimization of Maximum Mean Discrepancy (MMD)~\cite{long2015learning,long2016unsupervised}: the distributions of the learned source and target representations are forced to be as similar as possible by minimizing the distance between their mean embeddings.
The other strategy \cite{tzeng2015simultaneous,ganin2014unsupervised} relies on the so-called domain-confusion 
loss. This loss is introduced to learn an auxiliary classifier predicting if a sample comes from the source or from the target domain. Intuitively, by maximizing this term, \ie by imposing the auxiliary classifier to exhibit poor performance, domain-invariant features can be obtained.
Following these recent approaches, we present a domain adaptation method which simultaneously learns discriminative deep representations while being able to cope with domain shift in the unsupervised setting.
Differently from previous works, we do not focus on learning domain-invariant features by \emph{explicitly} optimizing additional loss terms (\eg MMD, domain-confusion).
We argue instead that different predictors should be used for source and target samples and that specific \textit{Domain Alignment} layers (\DALs) can be embedded into a deep architecture to align the observed data distributions to a canonical one.
Moreover, we depart from previous methods which decide \emph{a priori} which layers should be adapted and we endow our DA-layers with the ability to automatically learn the degree of alignment that should be pursued in each specific level of the network (Fig.\ref{fig:teaser}). This is to our knowledge the first work that tries to pursue this objective.
Finally, we propose to use the unlabeled target data to construct a prior distribution on the network parameters, biasing the learned solution towards models that are able to separate well the classes in the target domain.
%Finally, we show how, under certain conditions, our approach can be completely implemented by employing traditional layers, \ie batch normalization (BN, \cite{ioffe2015batch}) and the cross-entropy loss.
We call our algorithm DIAL -- DomaIn Alignment Layers. 
An extensive experimental evaluation, conducted on three publicly available datasets, demonstrates that DIAL greatly alleviates the domain discrepancy and outperforms state of the art techniques.
%Following recent successful approaches \cite{long2016unsupervised}, we present a novel method for unsupervised deep domain adaptation, which simultaneously align features from the source and the target domains and also learns deep representations by minimizing an entropy loss on target data. %, such as to reduce uncertainty of labeling the unlabeled data.
%Differently from previous works, in this paper we introduce a novel technique, inspired by batch normalization (BN) \cite{ioffe2015batch}, for aligning representations derived from the inner layers of a deep architecture. Batch normalization,
%\ie Z-normalization of internal CNN activations based on mini-batches, is commonly employed to reduce the internal covariate shift in deep networks. In this paper, we propose to revisit traditional BN  for deep domain adaptation and introduce a novel domain-aware BN technique. Our intuition is that, by adopting domain-specific mean and variance terms when applying BN to source and target samples, the domain discrepancy can be greatly alleviated. We demonstrate that, despite its simplicity, our approach outperforms state of the art techniques on publicly available datasets.

\begin{figure}
  \centering
%  \includegraphics[width=\columnwidth]{images/teaser-new.pdf}
  \caption{\DIAL learn a pair of transformations that shift the observed source and target distribution to match a desired reference distribution.}
  \label{fig:teaser}
\end{figure}

\textbf{Contributions}.
The contribution of this work is threefold.
First, we present an effective approach for unsupervised domain adaptation.
Our proposal is based on the introduction of DA-layers to explicitly address the domain shift problem. Our solution simultaneously aligns feature representations and learn where and to which extent adaptation should take place.  % without assuming the existence of a single predictor for source and target domains.
%Second, we show that, under certain assumptions, our method can be implemented by composing existing CNN layers.
Second, in contrast to previous works optimizing domain discrepancy regularization terms~\cite{long2016unsupervised,tzeng2015simultaneous,ganin2014unsupervised,long2015learning}, our DA-layers do not introduce any additional meta-parameters into the network.
Third, we perform an extensive experimental analysis on three different benchmarks.
We find that our unsupervised domain adaptation approach outperforms state-of-the-art methods and can be applied to different CNN architectures, consistently improving their performance in domain adaptation problems.
% The remaining of this paper is organized as follows. Section
% \ref{related} reviews previous work on unsupervised domain adaptation. The proposed
% method is introduced in Section \ref{} and experimental results are presented in Section \ref{}.
% Conclusions are drawn in Section \ref{}. 

==> method_o.tex <==
\label{method}
Let $\set X$ be the input space (\eg images) and $\set Y$ the output space (\eg image categories) of our learning task.
In unsupervised domain adaptation, we have a \emph{source} domain and a \emph{target} domain that
are identified via probability distributions $p^s_{\mathtt{xy}}$ and $p^t_\mathtt{xy}$, respectively, defined over $\set X\times\set Y$.
The two distributions are in general different and unknown, but we are provided with a source dataset $\set S=\{(x^s_1,y^s_1),\dots,(x^s_n,y^s_n)\}$ of \emph{i.i.d.} observations from $p^s_{\mathtt{xy}}$ and an unlabeled target dataset $\set T=\{x^t_1,\dots,x^t_m\}$ of \emph{i.i.d.} observations from the marginal $p^t_\mathtt x$.
The goal is to estimate a predictor from $\set S$ and $\set T$ that can be used to classify sample points from the target domain.
This task is particularly challenging because on one hand we lack direct observations of labels from the target domain and on the other hand the discrepancy between the source and target domain distributions prevents a predictor trained on $\set S$ to be readily applied to the target domain. 

A number of state of the art methods try to reduce the domain discrepancy by performing some form of alignment at the feature or classifier level. In particular, the recent, most successful methods try to \emph{couple} the training process and the domain adaptation step within \emph{deep} neural architectures~\cite{ganin2014unsupervised,long2016unsupervised,long2015learning}, as this solution enables alignments at different levels of abstraction. The approach we propose embraces the same philosophy, but
we depart from the majority of the methods 
%making the assumption that domain alignment can by pursued by applying the \emph{same} predictor to the source and target domains.  This is motivated by an impossibility theorem~\cite{ben2010impossibility}, which intuitively states that no learner relying on the \emph{covariate shift} hypothesis, \ie $p^s_{\mathtt y|\mathtt x}=p^t_{\mathtt y|\mathtt x}$,
%and achieving a low discrepancy between the source and target unlabeled distributions $p^s_\mathtt x$ and $p^t_\mathtt x$, 
%can succeed in domain adaptation without further relatedness assumptions between training and target distributions.
%For this reason, we assume that the source and target predictors are in general \emph{different} functions. Nonetheless, both predictors depend on a common parameter $\theta$ belonging to a set $\Theta$,  
%which couples explicitly the two predictors, but it is not directly involved in the alignment of the source and target domains. 
%This contrasts with the majority of state of the art methods 
that augment the loss function used to train their predictors with a regularization term penalizing discrepancies between source and target representations (see, \eg~\cite{ganin2014unsupervised,long2016unsupervised,long2015learning}). 
The perspective we take is different and is close in spirit to AdaBN~\cite{li2016revisiting}. It consists in hardcoding, in a sense, the desired domain-invariance properties into the source and target predictors through the introduction of so-called \emph{Domain-Alignment layers} (\DALs). Also, we distinguish from previous approaches in the field, by trying to sidestep the problem of deciding which layers should be aligned, and to what extent. We achieve this goal by endowing the architecture with the ability to \emph{automatically} tune the degree of alignment that should be considered in each domain-alignment layer. %This is to our knowledge the first work that tries to pursue this objective \samuel{\`E vero?}.
The rest of this section is devoted to providing the details of our method.

\subsection{Source and Target Predictors}
\label{sec:predictors}
The source and target predictors are implemented as two deep neural networks being almost identical, as they share the same structure and the same weights (given by the parameter $\theta$). However, the two networks contain also a number of special layers, the \DALs,
which implement a domain-specific operation.
Indeed, the role of such layers is to apply a data transformation
that aligns in a sense the observed input distribution with a reference distribution. 
Since in general the input distributions of the source and target predictors differ, while the reference distribution stays the same, we have that the two predictors undergo different transformations in the corresponding \DALs.
Consequently, the source and target predictors implement de facto different functions, which is important for the reasons given at the beginning of the section.

The actual implementation of our \DALs is inspired by AdaBN~\cite{li2016revisiting}, 
where Batch Normalization layers are used to independently align source and target distributions to a standard normal distribution, by matching the first- and second-order moments. The approach they propose is very simple as it merely consists in training using the source sample a network having BN-layers, thus obtaining the source predictor, and deriving the target predictor as a post-processing step, which re-estimates the BN statistics using target samples only. Accordingly, the source and target predictors share the same network parameters but have different BN statistics, thus rendering the two predictors different functions. 

The approach we propose sticks to the same idea of using BN-layers to align domains, but we introduce fundamental changes. One limitation of AdaBN is that the target samples have no influence on the network parameters, because they will trigger only an update of the BN statistics. Our approach overcomes this limitation by coupling the network parameters to both target and source samples at training time. This is achieved in two ways: first we introduce a prior distribution for the network parameters based on the target samples; second, we endow the architecture with the ability of learning the degree of adaptation by introducing a parametrized, cross-domain bias to the input distribution of each domain-specific \DAL. The rest of this subsection is devoted to describe the new layer, while we defer to the next subsection the description of the prior distribution.

\paragraph{\DAL.} As mentioned before, our \DAL is implemented using BN, but as opposed to its standard implementation, which computes first and second-order moments from the input distribution derived from the mini-batch, we let the latter statistics to be contaminated by samples from the other domain, thus introducing a cross-domain bias. 
Since the source and target predictors share the same network topology, each \DAL in one predictor has a matching \DAL in the other predictor. Let $x_s$ and $x_t$ denote inputs to matching \DALs in the source and target predictor, respectively, for a given feature channel and spatial location. Assume $q^s$ and $q^t$ to be the distribution of $x_s$ and $x_t$, respectively, and let $q_\alpha^{st}=\alpha q^s + (1-\alpha) q^t$ and, symmetrically, $q_\alpha^{ts}=\alpha q^t + (1-\alpha) q^s$ be cross-domain distributions mixed by a factor $\alpha\in[0.5,1]$. Then, the output of the \DALs in the source and target networks are given respectively by
\begin{equation}
\label{eqn:dal}
\mathtt {DA}(x_s;\alpha) = \frac{x_s-\mu_{st,\alpha}}{\sqrt{\epsilon+\sigma_{st,\alpha}^2}},\,\,\,
\mathtt {DA}(x_t;\alpha) = \frac{x_t-\mu_{ts,\alpha}}{\sqrt{\epsilon+\sigma_{ts,\alpha}^2}},
\end{equation}
where $\epsilon>0$ is a small number to avoid numerical issues in case of zero variance, $\mu_{st,\alpha}=\mathtt {E}_{x\sim q_\alpha^{st}}[x]$, $\sigma^2_{st,\alpha}=\mathtt {Var}_{x\sim q_\alpha^{st}}[x]$, and similarly $\mu_{ts,\alpha}$ and $\sigma^2_{st,\alpha}$ are mean and variance of $x\sim q^{ts}_\alpha$.
Akin to BN, we estimate the statistics based on the mini-batch and derive similarly the gradients through the statistics (see, Supplementary Material).


The rationale behind the introduction of the mixing factor $\alpha$ is that we can move from having an independent alignment of the two domains akin to AdaBN, when $\alpha=1$, to having a coupled normalization when $\alpha=0.5$.
In the former case the \DAL computes two different functions in the source and target predictors and is equivalent to considering a full degree of domain alignment. The latter case, instead, yields the same function since $q_{0.5}^{st}=q_{0.5}^{ts}$ thus transforming the two domains equally, which yields no domain-specific alignment.
Since the mixing parameter $\alpha$ is not fixed a priori but learned during the training phase, we obtain as a result that the network can decide how strong the domain alignment should be at each level of the architecture where \DAL is applied. More details about the actual CNN architectures used to implement the two domain predictors are given in Section~\ref{sec:setup}.

%To better understand how the domain-alignment transformation works, we consider a single \DAL in isolation.
%The desired output distribution, namely the reference distribution, is decided a priori and thus known.
%The input distribution instead is unknown, but we can rely on a sample $\set D$ thereof. Now given a transformation $g$ from a family of transformations $\set G$ we can push the reference distribution into the pre-image under $g$ via a variable change. This yields a family of distributions
%among which we can select the one, say $\hat g$, that most likely represents sample $\set D$.
%In other words, if $\mathtt v$ is a random variable following the reference distribution and we assume that the input observations in $\set D$ are realizations of random variable $\mathtt u=g^{-1}(\mathtt v)$, then we can determine the transformation $\hat g\in\set G$ as the one that maximizes the likelihood $p_\mathtt u(\set D|g)$.

%This idea paves the way to a number of transformations that could be obtained by playing with different reference distributions and families of transformations. However, in this work, we restrict our focus to a particular family of \DALs that we obtain by imposing the standard normal distribution as reference distribution and by considering channel-wise linear transformations, \ie $\set G=\{u\mapsto \diag au+b\,:\,a, b\in\mathbb R^d\}$ where $\diag a$ is a diagonal matrix with diagonal elements given by $a$. Under this setting, by pushing the reference distribution into the pre-image of $g\in\set G$ we obtain a normal distribution with mean $-\diag a^{-1}b$ and covariance $\diag a^{-2}$.
%The maximum likelihood estimate of $a$ and $b$ given sample $\set D$ yields $\diag a=\diag {\sigma (\set D)}^{-1}$ and $b=-\diag{ \sigma (\set D)}^{-1}\mu(\set D)$, where $\mu(\set D)$ and $\sigma(\set D)$ represent the sample mean and the square root of the diagonal of the sample covariance of $\set D$, respectively. The resulting domain-alignment transformation is $\hat g(u)=\diag{\sigma(\set D)}^{-1}\left[ u-\mu(\set D) \right]$. This transformation is not new in the context of deep networks, because it is equivalent to the well-known \emph{batch-normalization} layer~\cite{ioffe2015batch}, when $\set D$ is the mini-batch of a training iteration. Nevertheless, the way we use it for unsupervised domain adaptation is novel.\footnote{There is an unpublished work~\cite{li2016revisiting}, which is in parallel to ours, that uses batch normalization for \emph{a-posteriori} domain adaptation.}
%It is worth noting that other transformations could be explored, \eg the one we obtain by imposing a Laplace distribution as reference distribution, but we leave this as a potential future work.




%Since the \DALs require to estimate the domain-alignment transformation, we have to
%provide the source and target predictors with a domain sample at training time, which could correspond to the training set itself or a subset thereof (\eg mini-batch).
%In the rest of the section we denote by $f^\theta_y(x;x_\set S)$ the probability assigned by the source predictor with parameter $\theta$ to sample point $x$ for class label $y$, where $x_\set S=\{x_1^s,\dots,x_n^s\}$ is the source domain sample. Similarly, we write $f^\theta_y(x;x_\set T)$ 
%for the target predictor.\footnote{We use notation $x_\set T$ and $\set T$ interchangeably.}

%\samuel{Add properties of the layer, akin to BN}






\subsection{Training}\label{ss:training}
During the training phase we estimate the parameter $\theta$, which holds the neural network weights shared by the source and target predictors including the mixing factors pertaining to the \DALs, using the observations provided by the source dataset $\set S$ and the target dataset $\set T$. 
As we stick to a discriminative model, the unlabeled target dataset cannot be employed to express the data likelihood. However, we can exploit $\set T$ to construct a prior
distribution of the parameter $\theta$. Accordingly, we shape a posterior distribution of $\theta$ given the observations $\set S$ and $\set T$ as
\begin{equation}
    \pi(\theta|\set S,\set T)\propto\pi(y_{\set S}|x_{\set S},\set T,\theta)\pi(\theta|\set T, x_\set S)\,,%\prod_{(x,y)\in\set S}\pi(y|x,\theta)\,,
    \label{eq:posterior}
\end{equation}
where $y_{\set S}=\{y^s_1,\dots,y^s_n\}$ and $x_{\set S}=\{x^s_1,\dots,x^s_n\}$ collect the labels and data points of the observations in $\set S$, respectively.
The posterior distribution is maximized over $\Theta$ to obtain a maximum a posteriori estimate $\hat\theta$ of the parameter used in the source and target predictors:
\begin{equation}
    \hat\theta \in\argmax_{\theta\in\Theta} \pi(\theta|\set S,\set T)\,.
    \label{eq:MAP}
\end{equation}
The term $\pi(y_{\set S}|x_{\set S},\set T,\theta)$ in~\eqref{eq:posterior} represents the likelihood of $\theta$ with respect to the source dataset,
while
%given a sample $(x,y)$ from the source domain. This corresponds to \eg the $y$th output element of a neural network having a soft-max layer on top. The prior term 
$\pi(\theta|\set T, x_\set S)$ is the prior term depending on the target dataset, which acts as a regularizer in the classical learning theory sense. Both terms actually, depend on both domains due to the cross-domain statistics that we have in our \DALs for $\frac{1}{2}\leq\alpha<1$ and are estimated from samples from the source \emph{and} target domains.

The likelihood decomposes into the following product over sample points, due to the data sample \emph{i.i.d.} assumption:
\begin{equation}
    \pi(y_{\set S}|x_{\set S},\set T,\theta)=\prod_{i=1}^nf_s^\theta(y^s_i;x^s_i)\,,
    \label{eq:likelihood}
\end{equation}
where $f^\theta_s(y^s_i;x^s_i)$ is the probability that sample point $x^s_i$ takes label $y^s_i$ according to the source predictor (we omitted the dependence on $\set T$ and $x_\set S$ for notational convenience).

Before delving into the details of the prior term, we would like to remark on the absence of an explicit component in the probabilistic model that tries to align the source and target distributions.
This is because in our model the domain-alignment step is taken over by each predictor, independently, via the domain-alignment layers as shown in the previous subsection.

\paragraph{Prior distribution.}
The prior distribution of the parameter $\theta$ shared by the source and target predictors is constructed from the observed, target data distribution. This choice is motivated by the theoretical possibility of squeezing more bits of information from unlabeled data points insofar as they exhibit low levels of class overlap~\cite{oneill1978normal}. Accordingly, it is reasonable to bias a priori a predictor based on the degree of label uncertainty that is observed when the same predictor is applied to the target samples. Uncertainty in this sense can be measured for an hypothesis $\theta$ in terms of the empirical entropy of $\mathtt y|\theta$ conditioned on $\mathtt x$ as follows
\begin{equation}
    h(\theta|\set T,x_\set S)=-\frac{1}{m}\sum_{i=1}^m\sum_{y\in\set Y}f^\theta_t(y;x^t_i)\log f^\theta_t(y;x^t_i)\,,
    \label{eq:h}
\end{equation}
where $f_t(y;x^t_i)$ represents the probability that sample point $x_i^t$ takes label $y$ according to the target predictor (again we omitted the dependence on $\set T$ and $x_\set S$).

It is now possible to derive a prior distribution $\pi(\theta|\set T,x_\set S)$ in terms of the label uncertainty measure $h(\theta|\set T,\set x_\set S)$
by requiring the prior distribution to maximize the entropy under the constraint $\int h(\theta|\set T,x_\set S)\pi(\theta|\set T,x_\set S)d\theta=\varepsilon$, 
where the constant $\varepsilon>0$ specifies how small the label uncertainty should be on average. This yields a concave, variational optimization problem with solution:
\begin{equation}
    \pi(\theta|\set T,x_\set S)\propto\exp\left( -\lambda\, h(\theta|\set T,x_\set S) \right)\,,
    \label{eq:prior}
\end{equation}
where $\lambda$ is the Lagrange multiplier corresponding to $\varepsilon$. 
%This prior distribution has been introduced in the context of semi-supervised learning in~\cite{grandvalet2004semisupervised} and % and employed for unsupervised domain adaptation in~\cite{long2016unsupervised}.
The resulting prior distribution  
satisfies the desired property of preferring models that exhibit well separated classes (\ie having lower values of $h(\theta|\set T,x_\set S)$), thus enabling 
the exploitation of the information content of unlabeled target observations within a discriminative setting~\cite{grandvalet2004semisupervised}.

Prior distributions of this kind have been adopted also in other works~\cite{long2016unsupervised} in order to exploit more information from the target distribution, but has never been used before in conjunction to explicit domain alignment methods (\ie not based on additional regularization terms such as MMD and domain-confusion) like the one we are proposing.
%\elisa{motivation}

\paragraph{Inference.}
Once we have estimated the optimal network parameters $\hat\theta$ by solving~\eqref{eq:MAP}, we can remove the dependence of the target predictor on $\set T$ and $x_\set S$.
In fact, after fixing $\hat\theta$, the input distribution to each \DAL also becomes fixed, and we can thus compute and store the required statistics once at all, akin to standard BN. 

\subsection{Implementation Notes}
\DAL can be implemented as a mostly straightforward modification of standard Batch Normalization.
We refer the reader to the supplementary material for a complete derivation.
In our implementation in particular, we treat each pair of \DALs as a single network layer which simultaneously computes the two normalization functions in Equation~\eqref{eqn:dal} and learns the $\alpha$ parameter.
During training each batch contains a fixed number of source samples, followed by a fixed number of target samples, allowing our \DALs to simply differentiate between the two.
Similarly to standard BN, we keep separate moving averages of the source and target statistics.
Note that, as mentioned before, $\alpha \in [0.5,1]$.
We enforce this by clipping its value in the allowed range in each forward pass of the network.

By replacing the optimization problem in~\eqref{eq:MAP} with the equivalent minimization of the negative logarithm of $\pi(\theta|\set S, \set T)$ and combining \eqref{eq:posterior}, \eqref{eq:likelihood}, \eqref{eq:h} and \eqref{eq:prior} we obtain a loss function $L(\theta)=L^s(\theta) + \lambda L^t(\theta)$, where:
\begin{align*}
\label{eq:loss}
  L^s(\theta) &= - \frac{1}{n}\sum_{i=1}^n \log f_s^\theta(y_i^s;x_i^s)\,,\\
  L^t(\theta) &= - \frac{1}{m}\sum_{i=1}^m\sum_{y\in\set Y}f_t^\theta(y;x^t_i)\log f_t^\theta(y;x^t_i)\,.
\end{align*}
The term $L^s(\theta)$ is the standard log-loss applied to the source samples, while $L^t(\theta)$ is an entropy loss applied to the target samples.
The second term can be implemented by feeding $f_t^\theta(y;x^t_i)$ to both inputs of a cross-entropy loss layer, where supported by the deep learning toolkit of choice.
In our implementation, based on Caffe~\cite{jia2014caffe}, we obtain it by slightly modifying the existing \texttt{SoftmaxLoss} layer.
The code will be made publicly available.
